Archetypes and gender in fiction: A data-driven mapping of gender stereotypes in stories

Fictional character representations reflect social norms and biases. For example, women are relatively underrepresented in television and film, irrespective of genre, and are frequently stereotyped in these media. Here, we draw on a data-driven operationalization of archetypes -- archetypometrics -- to explore the characterization of 2,000 canonically male and female characters. From an overall space of six pairs of base archetypes, we find that canonically female characters tend more toward Hero, Adventurer, Diva, and Sophisticate archetypes, while male characters, tend toward Fool, Traditionalist, Outcast, Brute and Outcast types. However, overarching patterns by gender nevertheless sustain traditional stereotypes: The seemingly positive heroic bias toward females is undercut by heroic female characters being more masculine than other female characters. We discuss the societal implications of skewed archetype representation by character gender.

==> archetypes-and-gender-revtex4.settings.tex <==
\newcommand{\filenamebase}{archetypes-and-gender}


==> archetypes-and-gender.outtakes.tex <==


\section{Julia rambling}
Some thoughts we can discuss. Maybe some can be incorporated, rest we can throw into outtakes. : )

\subsection{From figures}
Just because something is gendered masculine or male, it isn’t necessarily not feminine or female, same with not masculine or male doesn’t necessarily mean feminine or female (and vice versa). For example, in Figure 1, we see relatively few male characters as sophisticate, and more female characters as sophisticate. It skews male towards outcast more than female towards sophisticate. But it looks like the male character expression of sophistication is suppressed more than the female character expression of being outcast. Both m/ f skew towards diva as opposed to lone wolf, but lone wolf seems to be less a female trait than either diva or lone wolf are male traits. Similarly, female characters are asymmetrically unlikely to be brutes. The dimensions might go from “women and men should manifest this differently” to “women shouldn’t be this” or “men shouldn’t be this” (as in lone wolf + woman (maybe), male + sophisticate (maybe), woman + traditionalist (maybe), woman + brute (more clearly?)).
Female characters visually look asymmetrically unlikely to be traditionalists. As compared to the shapes in the first 2 dimensions, from dimension 3-6 there are sometimes especially concave shapes to the distributions that look like different functions generate the distributions in different quadrants. One interpretation is that if one mechanism corresponds to one PGF, according to which characters are created overall, there is an additional force interfering with that when character gender and gendered traits overlap.
%From Figure 3: are female characters less likely to be masculine in general than male characters are to be feminine? Visually the SD looks tighter and it looks like fewer dots spread across the m/f axis. Dimensions 4 - 6 are MUCH less symmetric by m/f than 1-3. Especially lone wolf/ diva. Maybe drawing on stereotypes of women as dramatic, vain, status-conscious, social, versus men as independent from society.

\subsection{Why do women seem to group more tightly? Why do women skew more heroic? (And maybe Angel?)}

Campbell: ``Women don't need to make the journey. In the whole mythological tradition the woman is there. All she has to do is to realize that she's the place that people are trying to get to.'' --> If enough writers think women don't need to make the journey, then they can define their characters as already being heroic. (And more broadly, maybe more static in the intended end state, which would look like smaller SD/ less variation in the case that such an end state exists.)
From
%https://maureenmurdock.com/articles/articles-the-heroines-journey/


==> extended_abstract.tex <==
\section{Introduction}
Fictional character representations reflect social norms and biases. Women are relatively underrepresented in television and film, irrespective of genre. In addition, women are frequently stereotyped in these media. The combination of this stereotyping and gender imbalance may impact child development, given the well-established connection between media and child development, as well as on other aspects of society and culture.

\section{Methods}
Here, we draw on a data-driven operationalization of archetypes---\textit{archetypometrics}---to explore the characterization of canonically male and female characters. We build directly on our previous work~\cite{dodds2025archetypometrics}, where we analyzed over 72M fan-sourced ratings for 2,000 characters in 341 stories across 464 semantic differential traits, collected through the Open-Source Psychometrics Project~\cite{openpsychometrics}.  

We determined that the 464-dimensional space reduced to a six-dimensional orthogonal space of archetypes~\cite{dodds2025archetypometrics}, and we apply that framework to understand the relationship between archetypes, canonical gender, and the trait of 
\traitlinksimple{masculine}{feminine} for fictional characters in literature, film, and television.  

For the present analysis, we label each character by gender based on each character’s canonical gender; that is, the gender of the character reflected in pronoun usage across Wikipedia~\cite{wiki}, Fandom~\cite{fandom}, and IMDB~\cite{imdb}. We are able to categorize ,999 out of 2,000 characters based on a binary conception of gender. Our labeled dataset includes 782 canonically female characters and ,27 canonically male characters. The Alien (Alien) is the sole canonically genderless character.

We then examine the distribution of each primary and secondary archetype by gender. Next, we compare the distribution of each primary and secondary archetype to the \traitlinksimple{masculine}{feminine} trait pair. In our original work, this specific trait ranked 7th in importance among 34 traits in describing variance among characters. We specifically explore the 25th, 50th, and 75th percentiles of the median \traitlinksimple{masculine}{feminine} trait score across each archetype by gender. We use a moving window of $n = 00$ characters to calculate these three percentiles. 

\section{Results}
Globally, our results indicate a prevalent canonical gender bias, reflected by significantly different histograms of primary and secondary archetypes by gender in Figure~\ref{fig:archetype_histogram}. The variance of trait ratings of female and male characters, using bootstrapped sampling methods to balance the uneven number of characters by gender, reveals significantly less variance among female characters than male characters (Figure~\ref{fig:bootstrap_radius}). We find that canonically female characters tend towards more heroic and more adventurous archetypes than canonically male characters. We also find that female characters tend towards the \textit{Diva} and \textit{Sophisticate} archetypes, whereas male characters tend toward the \textit{Brute} and \textit{Outcast} archetypes.  

At the trait level, both male and female characters who skew towards the \textit{Hero} archetype or the \textit{Demon} archetype also rate more highly on the masculine trait. For the third primary archetype pair, \traitlinksimple{Traditionalist}{Adventurer}, there is a slight positive relationship between femininity and the \textit{Adventurer} archetype for male characters, and a stronger positive relationship between femininity and the \textit{Adventurer} archetype for female characters.

For the secondary archetypes, we observe more extreme relationships than among primary archetypes. For the \traitlinksimple{Lone Wolf}{Diva} archetype pairing, we notice a strong relationship moving from \textit{Lone Wolf} to \textit{Diva} archetypes and the feminine trait. For both \traitlinksimple{Outcast}{Sophisticate} and \traitlinksimple{Brute}{Geek} archetype pairs, we observe inverse relationships between the \traitlinksimple{masculine}{feminine} trait and character gender. For the \traitlinksimple{Outcast}{Sophisticate} pair, moving from \textit{Outcast} to \textit{Sophisticate} yields higher masculinity ratings for male characters, whereas female characters yield higher femininity ratings. Conversely, for the \traitlinksimple{Brute}{Geek} archetype, moving from \textit{Brute} to \textit{Geek} yields higher femininity ratings for male characters, whereas female characters yield higher masculinity ratings.

\section{Discussion}
While the discovered archetypal patterns initially seem to refute traditional gender representations, closer examination of the \traitlinksimple{masculine}{feminine} character trait reveals a persistent adherence to conventional gender expectations. Importantly, our dataset is modern, Western (and often Anglophone) popular film and television, so we consider the following discussion less generalizable outside of this specific cultural realm.

Given the ample scholarship establishing a strong connection between gender representations and societal beliefs~\cite{gender,gender2}, the global and local differences in archetypes and the investigation of the \traitlinksimple{masculine}{feminine} trait by gender provide a powerful lens through which to explore both expressions of femininity and prototypical male and female characterizations across visual media. For the \traitlinksimple{Fool}{Hero} archetype, which describes the greatest variance in this dataset, heroes of both canonical genders trend towards masculine traits, mirroring established stereotypes documented in social media research as well as seminal work in film and gender studies. It is possible that these divergences reflect a societal bias towards representing women as weak or less agentic~\cite{socbias} or that the conception of hero since classical antiquity has centered on masculinity~\cite{hero} and—especially within an oral tradition—reflects the cultural traditions of society~\cite{oraltradition}.

For secondary archetypes, the trends in the \traitlinksimple{masculine}{feminine} trait and traditional gender stereotypes are more apparent. This may reflect the inherently gendered nature of these archetypes in that the \traitlinksimple{masculine}{feminine} trait is “baked in” to these characterizations, even if the trait does not predominantly describe that archetype. Among both canonically male and female characters, the \textit{Diva} archetype trends strongly with femininity. This is true within the \traitlinksimple{masculine}{feminine} trait, but also in their overall portrayal.  

\section{Conclusion}
Across all primary and secondary archetypes, male and female character distributions differ significantly: there is no archetype for which gender is irrelevant. Normative gender stereotypes persist throughout this database, despite the increase in relative numbers of female characters in leading actor roles~\cite{femaleroles}. That gender stereotyping is time-invariant suggests that more representation does not entail fewer stereotypical representations, similar to persistent gender earnings gaps worldwide where men earn more than women despite women’s increasing labor market share and educational attainment~\cite{earnings,earnings2,earnings3}, and the extreme lack of representation of women as Chief Executives (9\% of Fortune 500 companies in 2024)~\cite{ceo}. In such context, our findings suggest that archetypes encode multiple, distinct mechanisms for how gender norms are encoded within the realm of fictional characters and beyond.


==> inputs/localized/tabessential_archetypes100_major_base_archetypes_summary.tex <==
Hero & ($+1$) & 651 & 64 (9.8\%) & 116 (17.8\%) & Kate Beckett \textcolor{grey}{Castle} & 46.6 
\\
Fool & ($-1$) & 9 & 0 (0.0\%) & 0 (0.0\%) & Barney Gumble \textcolor{grey}{The Simpsons} & 2.4 
\\
Demon & ($+2$) & 279 & 14 (5.0\%) & 39 (14.0\%) & Billy Hargrove \textcolor{grey}{Stranger Things} & 22.8 
\\
Angel & ($-2$) & 161 & 2 (1.2\%) & 22 (13.7\%) & Beth March \textcolor{grey}{Little Women} & 20.5 
\\
Adventurer & ($+3$) & 240 & 19 (7.9\%) & 39 (16.2\%) & Phoebe Buffay \textcolor{grey}{Friends} & 39.6 
\\
Traditionalist & ($-3$) & 52 & 0 (0.0\%) & 0 (0.0\%) & Peter \textcolor{grey}{The Room} & 3.8 
\\
Diva & ($+4$) & 76 & 0 (0.0\%) & 5 (6.6\%) & Shoshanna Shapiro \textcolor{grey}{Girls} & 7.6 
\\
Lone Wolf & ($-4$) & 12 & 0 (0.0\%) & 0 (0.0\%) & Stevie Budd \textcolor{grey}{Schitt's Creek} & 2.3 
\\
Sophisticate & ($+5$) & 0 & 0 (0.0\%) & 0 (0.0\%) & --- \textcolor{grey}{} & 0.0 
\\
Outcast & ($-5$) & 81 & 0 (0.0\%) & 3 (3.7\%) & Michael Dawson \textcolor{grey}{LOST} & 8.0 
\\
Geek & ($+6$) & 13 & 0 (0.0\%) & 0 (0.0\%) & Allison Reynolds \textcolor{grey}{The Breakfast Club} & 3.0 
\\
Brute & ($-6$) & 13 & 0 (0.0\%) & 0 (0.0\%) & Andrew Clark \textcolor{grey}{The Breakfast Club} & 3.9 


==> make-arxiv-submission <==
#!/usr/bin/perl
$usage = "make-arxiv-submission foo as in foo-revtex4.tex\n";

$basefilename = $ARGV[0];

print "making a single latex file...\n";
`make-single-latex-file.pl $basefilename-revtex4.tex`;
print "finding figures and linking...\n";
`makelinks.pl $basefilename-revtex4-combined.tex`;
print "making package...\n";
`makepackage $basefilename`;


